On-device Training: A First Overview on Existing Systems

The recent breakthroughs in machine learning (ML) and deep learning (DL) have catalyzed the design and development of various intelligent systems over wide application domains. While most existing machine learning models require large memory and computing power, efforts have been made to deploy some models on resource-constrained devices as well. A majority of the early application systems focused on exploiting the inference capabilities of ML and DL models, where data captured from different mobile and embedded sensing components are processed through these models for application goals such as classification and segmentation. More recently, the concept of exploiting the mobile and embedded computing resources for ML/DL model training has gained attention, as such capabilities allow (i) the training of models via local data without the need to share data over wireless links, thus enabling privacy-preserving computation by design, (ii) model personalization and environment adaptation, and (ii) deployment of accurate models in remote and hardly accessible locations without stable internet connectivity. This work targets to summarize and analyze state-of-the-art systems research that allows such on-device model training capabilities and provide a survey of on-device training from a systems perspective.

==> sections/8-futurework.tex <==
% \section{Future work}
% \label{sec:futurework}
% Our review shows that on-device training is feasible across all device types. We believe that on-device training holds the potential to enable a wide range of privacy-aware and infrastructure-independent personalized applications. However, fewer efforts have been made for highly constrained IoT devices, specifically at the scale of devices that feature only a couple hundred of memory and clock speeds in the sub-GHz range. Despite their significance in designing a wide range of smart applications, the lack of systems tailored for such platforms is mainly due to two reasons. Firstly, such constrained hardware gives less flexibility for system design. Secondly, there is no one-size-fits-all OS for these IoT devices; thus, it requires per-system/implementation optimization. Designing a common framework that enables per-platform customized \color{blue} on-device training \color{black} for resource-constraint IoT platforms can be an interesting direction for future research. Potentially, we can think of approaches such as (i) exploring the possibility of applying existing optimized techniques on tiny devices, (ii) designing specific efficient NN for tiny devices with considerations on both inference and training efficiency, and (iii) integrating ML features, both inference and training, on the OS level to ease future development and migration. Future research can be initiated by exploiting mature embedded OSes, such as Contiki~\cite{dunkels2004contiki}, FreeRTOS~\cite{barry2008freertos}, or Android Things~\cite{roy2020android}. 

